Lower large deviations for geometric functionals

This work develops a methodology for analyzing large-deviation lower tails associated with geometric functionals computed on a homogeneous Poisson point process. The technique applies to characteristics expressed in terms of stabilizing score functions exhibiting suitable monotonicity properties. We apply our results to clique counts in the random geometric graph, intrinsic volumes of Poisson-Voronoi cells, as well as power-weighted edge lengths in the random geometric, $k$-nearest neighbor and relative neighborhood graph.

==> gilb.tex <==
\section{Proofs}\label{sec-proofs}
\subsection{Proof of Theorem \ref{upThm}}
%
%UP BOUnD
%
\begin{proof}[Proof of Theorem \ref{upThm}, upper bound]
	Since $\xi^M$ is a bounded local observable, the contraction principle  and \cite[Theorem 3.1]{georgii2} give that
	$$\limsup_{n \to \infty} \frac1{n^d} \log \P(G_n \le a) \le \limsup_{n \to \infty} \frac1{n^d} \log \P(G_n^M \le a) \le -\inf_{\Q:\, \Q^o[\xi^M] \le a}h(\Q).$$
	Hence, it suffices to show that 
	$$\lim_{M \to \infty}\inf_{\Q:\, \Q^o[\xi^M] \le a}h(\Q) \ge \inf_{\Q:\, \Q^o[\xi] \le a}h(\Q).$$
	There exists a family of point processes $\{\Q_k\}_{k \ge 1}$ such that $\Q_k^o[\xi^k] \le a$ and such that
	$$\lim_{k \to \infty}h(\Q_k) = \lim_{M \to \infty}\inf_{\Q:\, \Q^o[\xi^M] \le a}h(\Q).$$
	Let $\Q_*$ be a subsequential limit of the $\{\Q_k\}_{k \ge 1}$. To simplify the presentation, we may assume that $\Q_*$ is the limit of $\{\Q_k\}_{k \ge 1}$.	Then, by monotone convergence,
		$$\Q_*^o[\xi] = \lim_{m \to \infty}\Q_*^o[\xi^m] = \lim_{m \to \infty}\lim_{k \to \infty}\Q_k^o[\xi^m]  \le a.$$
Since the specific relative entropy $h$ is lower semicontinuous, we arrive at 
		$$\liminf_{k \to \infty} h(\Q_k) \ge h(\Q_*) \ge \inf_{\Q:\, \Q^o[\xi] \le a}h(\Q),$$
		as asserted.
\end{proof}


%================================================
%================================================


\subsection{Proof of Theorem \ref{gilbThm}}

The proof of Theorem \ref{gilbThm} relies on the level-3 large deviation principle for the Poisson point process from \cite[Theorem 3.1]{georgii2}. However, since the score function is possibly unbounded, it is unclear in general whether $G_n$ depends continuously on the empirical process of the Poisson point process in the $\tau$-topology.

To establish  Theorem \ref{gilbThm}, we consider the truncation 
$$\xi^M(x, X) = \min\{\xi(x, X), M\}$$
of the original score function $\xi$ at a large threshold $M > 1$. Similarly, we put 
$$G_n^M = \frac1{n^d}\sum_{X_i \in X \cap Q_n} \xi^M(X_i, X).$$



%
%LOW BOUnD
%
The proof of the lower bound is more involved, since we can no longer rely on replacing $\P(G_n \le a)$ by $\P(G_n^M \le a)$. Instead, we use the sprinkling approach that has already been successfully applied in the setting of large deviations in wireless networks, see \cite{wireless2}. Loosely speaking, we construct a coupling that pushes away the Poisson point process from pathological regions, lying at the root of discontinuities.

	%
	%RARE DENSE LEM
	%
Sprinkling only works if the total number of points in pathological areas is small with high probability. To check this property, we say that a point $X_i \in X$ is \emph{$b$-dense} if $\#(B_r(X_i) \cap X) > b$ and write 
	$$N_{b, n} = \#\{X_i \in Q_n \text{ is $b$-dense}\}$$
	for the total number of $b$-dense points in $Q_n$. 
\begin{lemma}[Rareness of $b$-dense points]
	\label{rareDenseLem}
	Let $\de > 0$. Then,
$$		\limsup_{b \to \infty}\limsup_{n \to \infty}\frac1{n^d} \log \P(N_{b, n} > \de n^d) = -\infty.$$
\end{lemma}

%
%REM DENSE LEM
%
In the second step, we remove all $b$-dense points through the coupling. That is, we let $\Xm$ denote an independent thinning of $X$ with survival probability $1-\e$. Furthermore, we let $\Xp$ denote an independent Poisson point process with intensity $\e > 0$. Then, we define the coupled process 
	$$\Xe = \Xm \cup \Xp,$$
	which is again a Poisson point process with intensity 1 and we write $\P^\e$ for the probability measure associated with $\Xe$. 

	Now, let
	$$E_{b, n} = \{\Xp \cap Q_n = \es\} \cap \{\Xm \cap Q_n \text{ does not contain $b$-dense points}\}$$
	be the event that $\Xp$ does not contain points in $Q_n$ and that $\Xm$ does not contain any dense points in $Q_n$.
\begin{lemma}[Removal of $b$-dense points]
	\label{remDenseLem}
	Let $b, n, \e > 0$. Then, $\P$-almost surely, 
	$$\P^\e(E_{b,n}|X) \ge  \exp(-\e n^d + {N_{b, n}}\log(\e) ).$$
\end{lemma}

	%
	%MAIN THM
	%
Before establishing Lemmas \ref{rareDenseLem} and \ref{remDenseLem}, we illustrate how they enter the proof of \eqref{gilbLowEq}.
\begin{proof}[Proof of Theorem \ref{gilbThm}, lower bound]
	Let $M > 0$. Then, by \cite[Theorem 3.1]{georgii2},
	$$
	\liminf_{n \to \infty} \frac1{n^d} \log \P(G_n^M< a ) \ge  -\inf_{\Q:\, \Q^o[\xi^M] < a }h(\Q) \ge -\inf_{\Q:\, \Q^o[\xi] < a }h(\Q).
	$$
	Hence, it remains to show that 
	\begin{align}
	\label{gilbLowEq2}
	\liminf_{n \to \infty} \frac1{n^d} \log \P(G_n < a ) \ge \lim_{M \to \infty}\liminf_{n \to \infty} \frac1{n^d} \log \P(G_n^M < a ). 
	\end{align}
	
	%
	%COUP COnST
	%
	
	%
	%SPRINKL EQ
	%
	We note that since $\xi$ is increasing,
	$$\P^\e(G_n < a) \ge \P^\e(\{G_n^{M(b)} < a\} \cap E_{b, n} ) \ge \E\big[\one\{G_n^{M(b)} < a \}\P^\e[E_{b,n}|X]\big].$$
	Hence, by Lemma \ref{remDenseLem},
	\begin{align*}
		\P^\e(G_n < a)
		&\ge \exp(-\e n^d)\E\big[\one\{G_n^{M(b)} < a \}\e^{N_{b, n}}\big]\\
		&\ge \exp((\de \log(\e) - \e) n^d)\P(G_n^{M(b)} < a) - \P(N_{b, n} > \de n^d).
	\end{align*}
	Since $X$ and $\Xe$ share the same distribution, Lemma \ref{rareDenseLem} allows us to choose $b = b(\de) > 0$ sufficiently large such that 
	$$\liminf_{n \to \infty} \frac1{n^d}\log\P(G_n < a) \ge (\de \log(\e) - \e) + \liminf_{n \to \infty}\frac1{n^d} \log\P(G_n^{M(b)} < a).$$
	Hence, sending $b \to \infty$, $\e \to 0$ and $\de \to 0$ concludes the proof of \eqref{gilbLowEq2}.
\end{proof}


%
%PRF RARE DENSE
%
\begin{proof}[Proof of Lemma \ref{rareDenseLem}]
	Consider a sub-division of $Q_n$, for sufficiently large $n\in\N$, into sub-cubes $Q_a(z_i)=z_i+Q_a$ of side length $a>r$ where $z_i\in a\Z^d$. Put $N_i = \#(X \cap Q_a(z_i))$ the number of points in the $i$-th sub-cube and $N'_i =\#(X \cap Q_{2a}(z_i))$, the number of points the $i$-th sub-cube plus its adjacent sub-cubes. With these definitions, we have 
	$$N_{b,n}\le \sum_{i=1}^{(n/a)^d}N_i\one\{N'_i>b\}.$$
Then, by the exponential Markov inequality, for all $t> 0$, 
\begin{align*}
\log \P(N_{b, n} > \de n^d)&\le \log \P\Big(\sum_{i=1}^{(n/a)^d}N_i\one\{N'_i>b\}> \de n^d\Big)\le  -\de t n^d+\log \E\Big[\exp(t\sum_{i=1}^{(n/a)^d}N_i\one\{N'_i>b\})\Big].
\end{align*}
%		\log\P(\sum_i N_i \one\{N_i > b\} \ge \de n^d) \color{red} \le \color{black} n^d\Big(\log\Big(\E\Big[\exp(\de^{-1}N_0 \one\{N_0 > b\})\Big]\Big) - \color{red} 1 \color{black} \Big).
Now, note that the random variables $N_i\one\{N'_i>b\}$ and $N_j\one\{N'_j>b\}$ are independent whenever $\Vert z_i-z_j\Vert_\infty\ge 3$ and hence we have $3^d$ regular sub-grids of $a\Z^d$ containing mutually independent random variables $N_i\one\{N'_i>b\}$. Thus, using H\" older's inequality and independence, we have 
\begin{align*}
\log \E\Big[\exp(t\sum_{i=1}^{(n/a)^d}N_i\one\{N'_i>b\})\Big]\le \big(\frac{n}{3a}\big)^d\log \E\Big[\exp(3^dtN_o\one\{N'_o>b\})\Big],
\end{align*}
and it suffices to show that for all $t>0$, 
\begin{align*}
\limsup_{b \to \infty}\E\Big[\exp(3^dtN_o\one\{N'_o>b\})\Big]=1.
\end{align*}
But this follows from an application of the dominated convergence theorem. 
\end{proof}

%
%PRF REM DENSE
%
\begin{proof}[Proof of Lemma \ref{remDenseLem}]
	First, since $\Xp$ and $\Xm$ are independent, it suffices to compute 
	$$\P(\Xp \cap Q_n = \es\,|\,X)$$ and $$\P(\Xm \cap Q_n \text{ does not contain $b$-dense points}\,|\,X)$$ separately. The void probabilities for a Poisson point process give that $$\P(\Xp \cap Q_n = \es\,|\,X) = \exp(- \e n^d).$$ 
	Next, since $\Xm$ results from $X$ by an independent thinning with probability $\e$, we arrive at 
	$$\P(\Xm \cap Q_n \text{ does not contain $b$-dense points}\,|\,X) \ge \e^{N_{b, n}},$$
	as asserted.
\end{proof}

%================================================
%================================================

\subsection{Proof of Theorem \ref{neighbThm}}\label{sec-stabproof}

To prove Theorem \ref{neighbThm}, we consider the partition of $Q_n$ into $(n/M)^d$ subcubes of sidelength $M\ge 1$ and use sprinkling to regularize those subcubes that are not contained in the family $\akm$.  
%
%PRF
%
	%
	%XI-APPX
	%
	Let us write
	$$\xikm(\varphi) = \xi(\varphi \cap Q_{3M}) \wedge (C_0M^{d - \e_0})$$
	and define an approximation $\hkm$ of $H_n$ by replacing  $\xi(X - x)$ with $\xikm(X - x)$. 

	%
	%DEF COPULIGN
	%
	Similarly as before, we consider a coupling construction. Now, we let $\Xmm$ and $\Xpp$ denote an independent thinning of $X$ in $Q_n$ with survival probability $1 - M^{-d}$ and an independent Poisson point process with intensity $M^{-d}$, respectively. Then, 
	$$\Xee = \Xmm \cup \Xpp$$ 
	defines a unit-intensity Poisson point process.

	%
	%DEF events
	%
	In this coupling, we set 
	$$\ekm = \{\Xmm = X\} \cap \bigcap_{z \in \Z^d \cap Q_{n/M}} F_z^M,$$ 
	where $F_z^M$ denotes the following event. If $\max_{x \in X \cap Q_{M}(Mz)}R(X - x) > M$, then $\big((\Xpp-M(z+u)) \cap Q_M\big) \in \akm$ for every $u \in \Z^d \cap Q_{1}$. Otherwise, $\Xpp \cap Q_M(Mz) = \es$.
	In particular, leveraging condition {\bf (STAB)} and that $R$ is decreasing shows that
	$$H_n(\Xee) = \hkm(\Xee)$$
	holds in the event $\ekm$.
	As we shall prove below, the events $\ekm$ occur with a high probability.

	%
	%LOW COND PROB
	%
	\begin{lemma}\label{remreachinglem}
Let $M, n, \e>0$. Then, $\P$-almost surely, 
		\[\P(\ekm| X) \ge \exp(-M^{-d} n^d (2 + \log(p'_0))) \]
		for some $p'_0>0$
\end{lemma}
Before we prove Lemma~\ref{remreachinglem}, let us show how it implies Theorem~\ref{neighbThm}.
\begin{proof}[Proof of Theorem~\ref{neighbThm}]
Clearly, we have
\begin{align*}
		\hkm(\Xee) &= n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(\Xee - X_i) + n^{-d}\sum_{X_i \in \Xpp\cap Q_n} \xikm(\Xee - X_i).
\end{align*}
Using the almost-decreasingness of $\xi$, the second term on the right-hand side can be estimated as follows
\begin{align*}
& n^{-d} \sum_{X_i \in X \cap Q_n} (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \\
%\\ \leq & n^{-d} \sum_{X_i \in X \cap Q_n}  (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \sum_{j=1}^{N(M)} \mathds 1 \big\{ X_i \in \mathrm{Exc}(X_i,X^{M,j-1}) \big\}
&= n^{-d} \sum_{X_i \in X \cap Q_n}\sum_{j=1}^{N(M)} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\\
%&= n^{-d} \sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2 n^{-d}C_0M^{d - \e_0}\sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n}\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2k n^{-d}C_0M^{d - \e_0}N(M)
%&\le  n^{-d} \frac{n^d K_0 k}{M^d} C_0M^{d - \e_0}
\le 2K_0 k M^{-\eps_0}.
 \end{align*} 

By conditions {\bf (STAB)} and {\bf (FIN)}, the $R$-boundedness of $\xi$ implies that in the event $\ekm$,
	\begin{align*}
		\hkm(\Xee) &= n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(\Xee - X_i) + n^{-d}\sum_{X_i \in \Xpp\cap Q_n} \xikm(\Xee - X_i)\\
		&\le n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(X - X_i) +  2K_0 k M^{-\eps_0}+\frac1{M^d} K_0C_0M^{d - \e_0}  \\
		&\le \hkm(X)+  K_0(2k+C_0)M^{ - \e_0}.
	\end{align*}
	Hence, 
	\[\P(H_n(\Xee) < a) \ge \P(\{\hkm(\Xee) < a\} \cap \ekm) \ge \P(\{\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0}\} \cap \ekm).\numberthis\label{Hence}\]
	Conditioning on $X$ and applying Lemma \ref{remreachinglem} gives that 
	\begin{align*}
		\P(H_n(\Xee) < a) &\ge \E[\one\{\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0} \} \P(\ekm\, |\, X)] \\
		&\ge\P(\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0}) \exp(-M^{-d} n^d (2 + \log(p'_0))).
	\end{align*}
	Now, by \cite{georgii2}
	\begin{align*}
		\liminf_{n \to \infty}n^{-d}\log(\P(\hkm(X) < a -  (2k+C_0)K_0 M^{-\e_0})) \ge -\inf_{\Q:\, \Q^o[\xi^M] < a -  (2k+C_0)K_0 M^{-\e_0}} h(\Q).
	\end{align*}
	Finally, if $\Q$ is such that $\Q^o[\xi] < a$, then $\Q^o[\xi^M] < a - (C_0+2k)K_0 M^{-\e_0}$ for all sufficiently large $M$, so that
	$$\liminf_{M \to \infty} \Big( -\inf_{\Q:\, \Q^o[\xi^M] < a -  (2k+C_0)K_0 M^{-\e_0}} h(\Q) \Big) \ge -\inf_{\Q:\, \Q^o[\xi] < a}h(\Q),$$
	 as asserted.
\end{proof}

\begin{proof}[Proof of Lemma \ref{remreachinglem}]
	First, 
	$$\P(X = \Xmm) = \exp(-M^{-d}n^d).$$
	Second,
	$$\P(\Xpp \cap Q_M = \es) = \exp(-1).$$
	Third, by condition {(\bf PROB)} and independence
	$$\P\Big((\Xpp-Mu \cap Q_M) \in \akm \text{ for every }u \in \Z^d \cap Q_{1}\Big)=\P(\Xpp \cap Q_M \in \akm)^{2d+1}>p_0^{2d+1}=p'_0,$$
	Putting everything together concludes the proof.
\end{proof}



==> neighb.tex <==
\subsection{Proof of Theorem \ref{neighbThm}}\label{sec-stabproof}

To prove Theorem \ref{neighbThm}, we consider the partition of $Q_n$ into $(n/M)^d$ subcubes of sidelength $M\ge 1$ and use sprinkling to regularize those subcubes that are not contained in the family $\akm$.  
%
%PRF
%
	%
	%XI-APPX
	%
	Let us write
	$$\xikm(\varphi) = \xi(\varphi \cap Q_{3M}) \wedge (C_0M^{d - \e_0})$$
	and define an approximation $\hkm$ of $H_n$ by replacing  $\xi(X - x)$ with $\xikm(X - x)$. 

	%
	%DEF COPULIGN
	%
	Similarly as before, we consider a coupling construction. Now, we let $\Xmm$ and $\Xpp$ denote an independent thinning of $X$ in $Q_n$ with survival probability $1 - M^{-d}$ and an independent Poisson point process with intensity $M^{-d}$, respectively. Then, 
	$$\Xee = \Xmm \cup \Xpp$$ 
	defines a unit-intensity Poisson point process.

	%
	%DEF events
	%
	In this coupling, we set 
	$$\ekm = \{\Xmm = X\} \cap \bigcap_{z \in \Z^d \cap Q_{n/M}} F_z^M,$$ 
	where $F_z^M$ denotes the following event. If $\max_{x \in X \cap Q_{M}(Mz)}R(X - x) > M$, then $\big((\Xpp-M(z+u)) \cap Q_M\big) \in \akm$ for every $u \in \Z^d \cap Q_{1}$. Otherwise, $\Xpp \cap Q_M(Mz) = \es$.
	In particular, leveraging condition {\bf (STAB)} and that $R$ is decreasing shows that
	$$H_n(\Xee) = \hkm(\Xee)$$
	holds in the event $\ekm$.
	As we shall prove below, the events $\ekm$ occur with a high probability.

	%
	%LOW COND PROB
	%
	\begin{lemma}\label{remreachinglem}
Let $M, n, \e>0$. Then, $\P$-almost surely, 
		\[\P(\ekm| X) \ge \exp(-M^{-d} n^d (2 + \log(p'_0))) \]
		for some $p'_0>0$
\end{lemma}
Before we prove Lemma~\ref{remreachinglem}, let us show how it implies Theorem~\ref{neighbThm}.
\begin{proof}[Proof of Theorem~\ref{neighbThm}]
Clearly, we have
\begin{align*}
		\hkm(\Xee) &= n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(\Xee - X_i) + n^{-d}\sum_{X_i \in \Xpp\cap Q_n} \xikm(\Xee - X_i).
\end{align*}
Using the almost-decreasingness of $\xi$, the second term on the right-hand side can be estimated as follows
\begin{align*}
& n^{-d} \sum_{X_i \in X \cap Q_n} (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \\
%\\ \leq & n^{-d} \sum_{X_i \in X \cap Q_n}  (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \sum_{j=1}^{N(M)} \mathds 1 \big\{ X_i \in \mathrm{Exc}(X_i,X^{M,j-1}) \big\}
&= n^{-d} \sum_{X_i \in X \cap Q_n}\sum_{j=1}^{N(M)} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\\
%&= n^{-d} \sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2 n^{-d}C_0M^{d - \e_0}\sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n}\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2k n^{-d}C_0M^{d - \e_0}N(M)
%&\le  n^{-d} \frac{n^d K_0 k}{M^d} C_0M^{d - \e_0}
\le 2K_0 k M^{-\eps_0}.
 \end{align*} 

By conditions {\bf (STAB)} and {\bf (FIN)}, the $R$-boundedness of $\xi$ implies that in the event $\ekm$,
	\begin{align*}
		\hkm(\Xee) &= n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(\Xee - X_i) + n^{-d}\sum_{X_i \in \Xpp\cap Q_n} \xikm(\Xee - X_i)\\
		&\le n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(X - X_i) +  2K_0 k M^{-\eps_0}+\frac1{M^d} K_0C_0M^{d - \e_0}  \\
		&\le \hkm(X)+  K_0(2k+C_0)M^{ - \e_0}.
	\end{align*}
	Hence, 
	\[\P(H_n(\Xee) < a) \ge \P(\{\hkm(\Xee) < a\} \cap \ekm) \ge \P(\{\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0}\} \cap \ekm).\numberthis\label{Hence}\]
	Conditioning on $X$ and applying Lemma \ref{remreachinglem} gives that 
	\begin{align*}
		\P(H_n(\Xee) < a) &\ge \E[\one\{\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0} \} \P(\ekm\, |\, X)] \\
		&\ge\P(\hkm(X) < a - (2k+C_0)K_0 M^{-\e_0}) \exp(-M^{-d} n^d (2 + \log(p'_0))).
	\end{align*}
	Now, by \cite{georgii2}
	\begin{align*}
		\liminf_{n \to \infty}n^{-d}\log(\P(\hkm(X) < a -  (2k+C_0)K_0 M^{-\e_0})) \ge -\inf_{\Q:\, \Q^o[\xi^M] < a -  (2k+C_0)K_0 M^{-\e_0}} h(\Q).
	\end{align*}
	Finally, if $\Q$ is such that $\Q^o[\xi] < a$, then $\Q^o[\xi^M] < a - (C_0+2k)K_0 M^{-\e_0}$ for all sufficiently large $M$, so that
	$$\liminf_{M \to \infty} \Big( -\inf_{\Q:\, \Q^o[\xi^M] < a -  (2k+C_0)K_0 M^{-\e_0}} h(\Q) \Big) \ge -\inf_{\Q:\, \Q^o[\xi] < a}h(\Q),$$
	 as asserted.
\end{proof}

\begin{proof}[Proof of Lemma \ref{remreachinglem}]
	First, 
	$$\P(X = \Xmm) = \exp(-M^{-d}n^d).$$
	Second,
	$$\P(\Xpp \cap Q_M = \es) = \exp(-1).$$
	Third, by condition {(\bf PROB)} and independence
	$$\P\Big((\Xpp-Mu \cap Q_M) \in \akm \text{ for every }u \in \Z^d \cap Q_{1}\Big)=\P(\Xpp \cap Q_M \in \akm)^{2d+1}>p_0^{2d+1}=p'_0,$$
	Putting everything together concludes the proof.
\end{proof}


==> neighbproof.tex <==
\section{Proof of Theorem~\ref{Uneighbthm}}\label{sec-neighborproof}
\color{red} This section is aborted and should not be included in the main file. \color{black}
Note that almost every realization of $X$ is nonequidistant. The at most $k$ points $y \in \vp$ in Lemma~\ref{lemma-almostincreasing} that do not satisfy \eqref{NNdecrease} will be called the \emph{exceptional points} of $x$ in $\vp$, and the set of exceptional points of $x$ in $\vp$ will be denoted as $\mathrm{Exc}(x,\vp)$. Note that $\mathrm{Exc}(x,\vp) \subseteq k\mathrm{NN}(\vp \cup \{x\},x)$. %Hence, we have the bound
%\[ \xi(\vp \cup \{ x \} -y) - \xi(\vp - y) \leq \sup_{v \in Q_n \setminus \vp} R(\vp \cup \{ v \} - v)^{\alpha} \numberthis\label{incrementbound} \]
for any nonequidistant $\varphi \in \mathbf N$ and for any $x \in \vp$.

The part of the proof of Theorem~\ref{neighbThm} where the decreasingness of $\xi$ enters is the inequality \eqref{needsdecreasing}, which uses that the truncated score function
$$\xikm(\varphi) = \xi(\varphi \cap Q_{3M}) \wedge (C_0M^{d - \e_0})$$
is decreasing. This is certainly not true for our score function, but we can nevertheless provide a suitable alternative of the inequality \eqref{needsdecreasing} given that $0 \leq \alpha < d$.

Indeed, in the event $E_n^M$, the left-hand side of that inequality is 
\begin{align*}
		\hkm(\Xee) &= n^{-d}\sum_{X_i \in X\cap Q_n} \xikm(\Xee - X_i) + n^{-d}\sum_{X_i \in \Xpp\cap Q_n} \xikm(\Xee - X_i), \numberthis\label{oldfirstline} \end{align*}
where each quantity is defined according to Section~\ref{sec-stabproof} with $\xi$ defined in \eqref{xineighbordef}. 
Let us write
\begin{align*}
n^{-d}& \sum_{X_i \in X\cap Q_n}  \xikm(\Xee - X_i) =  n^{-d}\sum_{X_i \in X\cap Q_n}  \xi^M(X - X_i)  \numberthis\label{oldfirstterm}
\\ & \qquad + n^{-d} \sum_{X_i \in X \cap Q_n} (\xikm(\Xee - X_i)  -\xikm(X-X_i)).
%\\ &  \leq  n^{-d}\sum_{X_i \in X\cap Q_n} \xi^M(X - X_i) + n^{-d} \sum_{X_j \in X^M \setminus X} \sum_{X_i \in \mathrm{Exc}(X_j,\varphi)} (\xikm(\Xee - X_i)  -\xikm(X-X_i)) 
%\\ &  \leq  n^{-d}\sum_{X_i \in X\cap Q_n} \xi^M(X - X_i) + n^{-d} M^d K_0 k \sup_{X_i \in X \cap Q_n}  (\xikm(\Xee - X_i)  -\xikm(X-X_i)).
\end{align*}
Using Lemma~\ref{lemma-almostincreasing}, let us now estimate in the event $E_n^M$ the second term on the right-hand side as follows. Let $(Y_i)_{i=1}^{N(M)}$ be an arbitrary enumeration of $X^M \setminus X$. In the event $E_n^M$, we have that $N(M) \leq n^d K_0/M^d$. For $j = 0,\ldots,N(M)$, let us write $X^{M,j}=X \cup \{ Y_1,\ldots,Y_j \}$; then $X^{M,0}=X$ and $X^{M,N(M)} = X^M$. Now, Lemma~\ref{lemma-almostincreasing} implies

\begin{align*}
& n^{-d} \sum_{X_i \in X \cap Q_n} (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \\
%\\ \leq & n^{-d} \sum_{X_i \in X \cap Q_n}  (\xikm(\Xee - X_i)  -\xikm(X-X_i)) \sum_{j=1}^{N(M)} \mathds 1 \big\{ X_i \in \mathrm{Exc}(X_i,X^{M,j-1}) \big\}
&= n^{-d} \sum_{X_i \in X \cap Q_n}\sum_{j=1}^{N(M)} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\\
%&= n^{-d} \sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n} (\xikm(X^{M,j}) - X_i)  -\xikm(X^{M,j-1})-X_i))\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2 n^{-d}C_0M^{d - \e_0}\sum_{j=1}^{N(M)}\sum_{X_i \in X \cap Q_n}\one\{\xikm(X^{M,j}) - X_i) >\xikm(X^{M,j-1})-X_i)\}\\
&\le 2k n^{-d}C_0M^{d - \e_0}N(M)
%&\le  n^{-d} \frac{n^d K_0 k}{M^d} C_0M^{d - \e_0}
\le 2K_0 k M^{-\eps_0}.
 \end{align*} 
 The right-hand side tends to zero as $M \to \infty$. Further, the first term on the right-hand side of \eqref{oldfirstline} as well as the first term on the right-hand side of \eqref{oldfirstterm} can be handled analogously to the proof of Theorem~\ref{neighbThm}. Hence,
 $$\P(H_n(\Xee) < a) \ge \P(\{\hkm(\Xee) < a\} \cap \ekm) \ge \P(\{\hkm(X) < a - K_0(k+C_0) M^{-\eps_0}\} \cap \ekm).$$ 
This right-hand side is the same as the one of \eqref{Hence}, up to the prefactor of $K_0 M^{-\eps_0}$, which tends to zero as $M \to \infty$. Hence, the proof of Theorem~\ref{Uneighbthm} can be completed analogously to the one of Theorem~\ref{neighbThm}.

